SemEval-2024 Task 1: Semantic Textual Relatedness for African and Asian Languages

We present the first shared task on Semantic Textual Relatedness (STR). While earlier shared tasks primarily focused on semantic similarity, we instead investigate the broader phenomenon of semantic relatedness across 14 languages: Afrikaans, Algerian Arabic, Amharic, English, Hausa, Hindi, Indonesian, Kinyarwanda, Marathi, Moroccan Arabic, Modern Standard Arabic, Punjabi, Spanish, and Telugu. These languages originate from five distinct language families and are predominantly spoken in Africa and Asia -- regions characterised by the relatively limited availability of NLP resources. Each instance in the datasets is a sentence pair associated with a score that represents the degree of semantic textual relatedness between the two sentences. Participating systems were asked to rank sentence pairs by their closeness in meaning (i.e., their degree of semantic relatedness) in the 14 languages in three main tracks: (a) supervised, (b) unsupervised, and (c) crosslingual. The task attracted 163 participants. We received 70 submissions in total (across all tasks) from 51 different teams, and 38 system description papers. We report on the best-performing systems as well as the most common and the most effective approaches for the three different tracks.

==> tables/data_splits.tex <==
\begin{table*}[h]
    \centering
    \small
   % \begin{tabular}{ccccccccccccccc}
     \begin{tabular}{lrrrrrrrrrrrrr}
        \toprule[1.2pt]
         %& \multicolumn{14}{c}{\textbf{Languages}} \\
        %\cmidrule(lr){2-15}
         \textbf{Data}& \texttt{afr} & \texttt{amh} & \texttt{arb} & \texttt{arq} & \texttt{ary} & \texttt{eng} & \texttt{esp} & \texttt{hau} & \texttt{hin} & \texttt{ind} & \texttt{kin} & \texttt{mar} & \texttt{tel}  \\
        \midrule
        \textbf{Train}& - & 992 & - & 1,262 & 925 & 5,500 & 1,562 & 1,763 & - & - & 778 & 1,155 & 1,146  \\
     %   \midrule
        \textbf{Dev}& 375 & 95 & 32 & 92 & 70 & 250 & 140 & 212 & 288 & 144 & 102 & 293& 130  \\
      %  \midrule
        \textbf{Test}& 375 & 171 & 595 & 584 & 427 & 2,500 & 600 & 603 & 968 & 360 & 222 & 298 & 297  \\ \midrule
        \textbf{Total} & 750& 1,258 & 627 & 1,938 & 1,422 & 8,250 & 2,299 & 2,578 & 1,256 & 504 & 1,102 & 1,746 & 1,573 \\
        \bottomrule
    \end{tabular}
    \caption{Number of instances in the training, dev, and test sets for the different datasets. The languages with no training data (\texttt{afr, arb, hin, ind}) were only used in unsupervised and cross-lingual settings.}
    \label{tab:data_splits}
    \vspace*{-3mm}
\end{table*}


==> tables/data_table.tex <==
\begin{table*}[h]
\small
\centering
    \begin{tabular}{lll}
    \toprule[1.2pt]
        \textbf{Lang.} & \textbf{Curation technique} & \textbf{Data Sources} \\ \midrule
        \texttt{afr} & Overlap, Random selection, Manual check & News data, reviews, recipes, blogs.\\
        \texttt{amh} & Overlap & Wikipedia, CommonCrawl, other. \\
        \texttt{arb} & Overlap, Contiguity, Random selection, Manual check& Ted talk subtitles, news data. \\
        \texttt{arq} & Overlap, Contiguity, Random selection, Manual check & YouTube comments, conversational data.\\
        \texttt{ary} & Overlap &News data\\
        \texttt{eng} & Overlap, Similarity, Paraphrases, Contiguity, Randomness& Book reviews, news data, tweets, other.\\
        \texttt{esp} & Overlap, Contiguity, Similarity & Movie reviews, news data, other.\\
        \texttt{hau} & Overlap& News data\\
        \texttt{hin} & Overlap, Paraphrase generation &News headlines \\
        \texttt{ind} & Overlap &Wikipedia, news data.\\
        \texttt{kin} & Overlap & News data. \\
        \texttt{mar} & Overlap, Paraphrase generation & News headlines\\
        \texttt{pan} & Overlap & News headlines Varta dataset \cite{aralikatte-etal-2023-varta}\\
        \texttt{tel} & Overlap, Paraphrase generation &News eadlines\\ \bottomrule
    \end{tabular}
\caption{The curation techniques used for data creation. We list the main textual sources present in the datasets we used to pair our sentences. More details are shared in Section \ref{sec:dataset_curation}.}
\label{tab:data_collection}
\end{table*}
% \documentclass[10pt, a4paper]{article}
% \usepackage{booktabs} % For professional-quality tables

% ... (other packages and settings)

 % eng  & & \citet{rao-tetreault-2018-dear, wan2018item} \\
          %  & & \citet{bowman-etal-2015-large,wieting2017paranmt} 

       %   yang-etal-2019-paws,araujo2022evaluation, huertastato2021silt
